The isomorphism problem for Grassmannian Schubert varieties

We prove that Schubert varieties in potentially different Grassmannians are isomorphic as varieties if and only if their corresponding Young diagrams are identical up to a transposition. We also discuss a generalization of this result to Grassmannian Richardson varieties. In particular, we prove that Richardson varieties in potentially different Grassmannians are isomorphic as varieties if their corresponding skew diagrams are semi-isomorphic as posets, and we conjecture the converse. Here, two posets are said to be semi-isomorphic if there is a bijection between their sets of connected components such that the corresponding components are either isomorphic or opposite.

==> references.tex <==
\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
\begin{thebibliography}{10}

\bibitem{anderson.chen:equivariant}
D.~Anderson and L.~Chen, \emph{Equivariant quantum {S}chubert polynomials},
  Adv. Math. \textbf{254} (2014), 300--330. \MR{3161101}

\bibitem{anderson.chen:positivity}
\bysame, \emph{Positivity of equivariant {G}romov-{W}itten invariants}, Math.
  Res. Lett. \textbf{22} (2015), no.~1, 1--9. \MR{3342175}

\bibitem{anderson.chen.ea:quantum}
D.~Anderson, L.~Chen, and H.-H. Tseng, \emph{The quantum {$K$}-theory of a
  homogeneous space is finite}, arXiv:1804.04579.

\bibitem{bertram:quantum}
A.~Bertram, \emph{Quantum {S}chubert calculus}, Adv. Math. \textbf{128} (1997),
  no.~2, 289--305. \MR{1454400 (98j:14067)}

\bibitem{bertram.ciocan-fontanine.ea:quantum}
A.~Bertram, I.~Ciocan-Fontanine, and W.~Fulton, \emph{Quantum multiplication of
  {S}chur polynomials}, J. Algebra \textbf{219} (1999), no.~2, 728--746.
  \MR{1706853 (2000k:14042)}

\bibitem{buch:quantum}
A.~S. Buch, \emph{Quantum cohomology of {G}rassmannians}, Compositio Math.
  \textbf{137} (2003), no.~2, 227--235. \MR{1985005}

\bibitem{buch:mutations}
\bysame, \emph{Mutations of puzzles and equivariant cohomology of two-step flag
  varieties}, Ann. of Math. (2) \textbf{182} (2015), no.~1, 173--220.
  \MR{3374959}

\bibitem{buch.chaput.ea:finiteness}
A.~S. Buch, P.-E. Chaput, L.~C. Mihalcea, and N.~Perrin, \emph{Finiteness of
  cominuscule quantum {$K$}-theory}, Ann. Sci. \'{E}c. Norm. Sup\'{e}r. (4)
  \textbf{46} (2013), no.~3, 477--494 (2013). \MR{3099983}

\bibitem{buch.chaput.ea:chevalley}
\bysame, \emph{A {C}hevalley formula for the equivariant quantum {$K$}-theory
  of cominuscule varieties}, Algebr. Geom. \textbf{5} (2018), no.~5, 568--595.
  \MR{3847206}

\bibitem{buch.chaput.ea:projected}
\bysame, \emph{Projected {G}romov-{W}itten varieties in cominuscule spaces},
  Proc. Amer. Math. Soc. \textbf{146} (2018), no.~9, 3647--3660. \MR{3825822}

\bibitem{buch.chung.ea:euler}
A.~S. Buch, S.~Chung, C.~Li, and L.~C. Mihalcea, \emph{Euler characteristics in
  the quantum {$K$}-theory of flag varieties}, Selecta Math. (N.S.) \textbf{26}
  (2020), no.~2, Paper No. 29, 11. \MR{4083680}

\bibitem{buch.kresch.ea:puzzle}
A.~S. Buch, A.~Kresch, K.~Purbhoo, and H.~Tamvakis, \emph{The puzzle conjecture
  for the cohomology of two-step flag manifolds}, J. Algebraic Combin.
  \textbf{44} (2016), no.~4, 973--1007. \MR{3566227}

\bibitem{buch.kresch.ea:gromov-witten}
A.~S. Buch, A.~Kresch, and H.~Tamvakis, \emph{Gromov-{W}itten invariants on
  {G}rassmannians}, J. Amer. Math. Soc. \textbf{16} (2003), no.~4, 901--915.
  \MR{1992829}

\bibitem{buch.kresch.ea:quantum}
\bysame, \emph{Quantum {P}ieri rules for isotropic {G}rassmannians}, Invent.
  Math. \textbf{178} (2009), no.~2, 345--405. \MR{2545685}

\bibitem{buch.kresch.ea:giambelli}
\bysame, \emph{A {G}iambelli formula for even orthogonal {G}rassmannians}, J.
  Reine Angew. Math. \textbf{708} (2015), 17--48. \MR{3420327}

\bibitem{buch.kresch.ea:giambelli*1}
\bysame, \emph{A {G}iambelli formula for isotropic {G}rassmannians}, Selecta
  Math. (N.S.) \textbf{23} (2017), no.~2, 869--914. \MR{3624902}

\bibitem{buch.mihalcea:quantum}
A.~S. Buch and L.~C. Mihalcea, \emph{Quantum {$K$}-theory of {G}rassmannians},
  Duke Math. J. \textbf{156} (2011), no.~3, 501--538. \MR{2772069}

\bibitem{chaput.manivel.ea:quantum*1}
P.-E. Chaput, L.~Manivel, and N.~Perrin, \emph{Quantum cohomology of minuscule
  homogeneous spaces}, Transform. Groups \textbf{13} (2008), no.~1, 47--89.
  \MR{2421317 (2009e:14095)}

\bibitem{chaput.manivel.ea:affine}
\bysame, \emph{Affine symmetries of the equivariant quantum cohomology ring of
  rational homogeneous spaces}, Math. Res. Lett. \textbf{16} (2009), no.~1,
  7--21. \MR{2480556 (2010h:14086)}

\bibitem{ciocan-fontanine:quantum}
I.~Ciocan-Fontanine, \emph{Quantum cohomology of flag varieties}, Internat.
  Math. Res. Notices (1995), no.~6, 263--277. \MR{1344348 (96h:14071)}

\bibitem{ciocan-fontanine:quantum*2}
\bysame, \emph{On quantum cohomology rings of partial flag varieties}, Duke
  Math. J. \textbf{98} (1999), no.~3, 485--524. \MR{1695799 (2000d:14058)}

\bibitem{fomin.gelfand.ea:quantum}
S.~Fomin, S.~Gelfand, and A.~Postnikov, \emph{Quantum {S}chubert polynomials},
  J. Amer. Math. Soc. \textbf{10} (1997), no.~3, 565--596. \MR{1431829
  (98d:14063)}

\bibitem{fulton:young}
W.~Fulton, \emph{Young tableaux}, London Mathematical Society Student Texts,
  vol.~35, Cambridge University Press, Cambridge, 1997, With applications to
  representation theory and geometry. \MR{1464693}

\bibitem{fulton:private}
\bysame, private communication, 2001.

\bibitem{fulton.pandharipande:notes}
W.~Fulton and R.~Pandharipande, \emph{Notes on stable maps and quantum
  cohomology}, Algebraic geometry---{S}anta {C}ruz 1995, Proc. Sympos. Pure
  Math., vol.~62, Amer. Math. Soc., Providence, RI, 1997, pp.~45--96.
  \MR{1492534}

\bibitem{fulton.woodward:quantum}
W.~Fulton and C.~Woodward, \emph{On the quantum product of {S}chubert classes},
  J. Algebraic Geom. \textbf{13} (2004), no.~4, 641--661. \MR{2072765}

\bibitem{givental:wdvv}
A.~Givental, \emph{On the {WDVV} equation in quantum {$K$}-theory}, Michigan
  Math. J. \textbf{48} (2000), 295--304, Dedicated to William Fulton on the
  occasion of his 60th birthday. \MR{1786492 (2001m:14078)}

\bibitem{givental.kim:quantum}
A.~Givental and B.~Kim, \emph{Quantum cohomology of flag manifolds and {T}oda
  lattices}, Comm. Math. Phys. \textbf{168} (1995), no.~3, 609--641.
  \MR{1328256 (96c:58027)}

\bibitem{gorbounov.korff:quantum}
V.~Gorbounov and C.~Korff, \emph{Quantum integrability and generalised quantum
  {S}chubert calculus}, Adv. Math. \textbf{313} (2017), 282--356. \MR{3649227}

\bibitem{hiller.boe:pieri}
H.~Hiller and B.~Boe, \emph{Pieri formula for {${\rm SO}_{2n+1}/{\rm U}_n$} and
  {${\rm Sp}_n/{\rm U}_n$}}, Adv. in Math. \textbf{62} (1986), no.~1, 49--67.
  \MR{859253 (87k:14058)}

\bibitem{huang.li:equivariant}
Y.~Huang and C.~Li, \emph{On equivariant quantum {S}chubert calculus for
  {$G/P$}}, J. Algebra \textbf{441} (2015), 21--56. \MR{3391918}

\bibitem{iritani.milanov.ea:reconstruction}
H.~Iritani, T.~Milanov, and V.~Tonita, \emph{Reconstruction and convergence in
  quantum {$K$}-theory via difference equations}, Int. Math. Res. Not. IMRN
  (2015), no.~11, 2887--2937. \MR{3373040}

\bibitem{kato:frobenius}
S.~Kato, \emph{Frobenius splitting of {S}chubert varieties of semi-infinite
  flag manifolds}, arXiv:1810.07106.

\bibitem{kato:loop}
\bysame, \emph{Loop structure on equivariant {$K$}-theory of semi-infinite flag
  manifolds}, arXiv:1805.01718.

\bibitem{kim:quantum}
B.~Kim, \emph{Quantum cohomology of partial flag manifolds and a residue
  formula for their intersection pairings}, Internat. Math. Res. Notices
  (1995), no.~1, 1--15 (electronic). \MR{1317639 (96c:58028)}

\bibitem{kim:equivariant}
\bysame, \emph{On equivariant quantum cohomology}, Internat. Math. Res. Notices
  (1996), no.~17, 841--851. \MR{1420551 (98h:14013)}

\bibitem{kim:quantum*1}
\bysame, \emph{Quantum cohomology of flag manifolds {$G/B$} and quantum {T}oda
  lattices}, Ann. of Math. (2) \textbf{149} (1999), no.~1, 129--148.
  \MR{1680543 (2001c:14081)}

\bibitem{kontsevich.manin:gromov-witten}
M.~Kontsevich and Yu. Manin, \emph{Gromov-{W}itten classes, quantum cohomology,
  and enumerative geometry}, Comm. Math. Phys. \textbf{164} (1994), no.~3,
  525--562. \MR{1291244 (95i:14049)}

\bibitem{kresch.tamvakis:quantum}
A.~Kresch and H.~Tamvakis, \emph{Quantum cohomology of the {L}agrangian
  {G}rassmannian}, J. Algebraic Geom. \textbf{12} (2003), no.~4, 777--810.
  \MR{1993764 (2004h:14063)}

\bibitem{kresch.tamvakis:quantum*1}
\bysame, \emph{Quantum cohomology of orthogonal {G}rassmannians}, Compos. Math.
  \textbf{140} (2004), no.~2, 482--500. \MR{2027200 (2005d:14080)}

\bibitem{lam.li.ea:conjectural}
T.~Lam, C.~Li, L.~C. Mihalcea, and M.~Shimozono, \emph{A conjectural {P}eterson
  isomorphism in {$K$}-theory}, J. Algebra \textbf{513} (2018), 326--343.
  \MR{3849889}

\bibitem{lee:quantum*1}
Y.-P. Lee, \emph{Quantum {$K$}-theory. {I}. {F}oundations}, Duke Math. J.
  \textbf{121} (2004), no.~3, 389--424. \MR{2040281 (2005f:14107)}

\bibitem{lenart.maeno:quantum}
C.~Lenart and T.~Maeno, \emph{Quantum {G}rothendieck polynomials},
  math.CO/0608232.

\bibitem{lenart.postnikov:affine}
C.~Lenart and A.~Postnikov, \emph{Affine {W}eyl groups in {$K$}-theory and
  representation theory}, Int. Math. Res. Not. IMRN (2007), no.~12, Art. ID
  rnm038, 65. \MR{2344548}

\bibitem{macdonald:symmetric*1}
I.~G. Macdonald, \emph{Symmetric functions and {H}all polynomials}, second ed.,
  Oxford Mathematical Monographs, The Clarendon Press Oxford University Press,
  New York, 1995, With contributions by A. Zelevinsky, Oxford Science
  Publications. \MR{1354144 (96h:05207)}

\bibitem{manivel:symmetric}
L.~Manivel, \emph{Symmetric functions, {S}chubert polynomials and degeneracy
  loci}, SMF/AMS Texts and Monographs, vol.~6, American Mathematical Society,
  Providence, RI, 2001, Translated from the 1998 French original by John R.
  Swallow, Cours Sp{\'e}cialis{\'e}s [Specialized Courses], 3. \MR{1852463
  (2002h:05161)}

\bibitem{matsumura:commutative*1}
H.~Matsumura, \emph{Commutative ring theory}, second ed., Cambridge Studies in
  Advanced Mathematics, vol.~8, Cambridge University Press, Cambridge, 1989,
  Translated from the Japanese by M. Reid. \MR{1011461}

\bibitem{mihalcea:positivity}
L.~C. Mihalcea, \emph{Positivity in equivariant quantum {S}chubert calculus},
  Amer. J. Math. \textbf{128} (2006), no.~3, 787--803. \MR{2230925}

\bibitem{mihalcea:equivariant*1}
\bysame, \emph{On equivariant quantum cohomology of homogeneous spaces:
  {C}hevalley formulae and algorithms}, Duke Math. J. \textbf{140} (2007),
  no.~2, 321--350. \MR{2359822}

\bibitem{mihalcea:giambelli}
\bysame, \emph{Giambelli formulae for the equivariant quantum cohomology of the
  {G}rassmannian}, Trans. Amer. Math. Soc. \textbf{360} (2008), no.~5,
  2285--2301. \MR{2373314}

\bibitem{propp.roby:homomesy}
J.~Propp and T.~Roby, \emph{Homomesy in products of two chains}, Electron. J.
  Combin. \textbf{22} (2015), no.~3, Paper 3.4, 29. \MR{3367853}

\bibitem{ruan.tian:mathematical}
Y.~Ruan and G.~Tian, \emph{A mathematical theory of quantum cohomology}, Math.
  Res. Lett. \textbf{1} (1994), no.~2, 269--278. \MR{1266766 (95b:58025)}

\bibitem{seidel:1}
P.~Seidel, \emph{{$\pi_1$} of symplectic automorphism groups and invertibles in
  quantum homology rings}, Geom. Funct. Anal. \textbf{7} (1997), no.~6,
  1046--1095. \MR{1487754}

\bibitem{siebert.tian:quantum}
B.~Siebert and G.~Tian, \emph{On quantum cohomology rings of {F}ano manifolds
  and a formula of {V}afa and {I}ntriligator}, Asian J. Math. \textbf{1}
  (1997), no.~4, 679--695. \MR{1621570 (99d:14060)}

\bibitem{witten:verlinde}
E.~Witten, \emph{The {V}erlinde algebra and the cohomology of the
  {G}rassmannian}, Geometry, topology, \& physics, Conf. Proc. Lecture Notes
  Geom. Topology, IV, Int. Press, Cambridge, MA, 1995, pp.~357--422.
  \MR{1358625 (98c:58016)}

\bibitem{woodward:d}
C.~T. Woodward, \emph{On {D}. {P}eterson's comparison formula for
  {G}romov-{W}itten invariants of {$G/P$}}, Proc. Amer. Math. Soc. \textbf{133}
  (2005), no.~6, 1601--1609. \MR{2120266}

\end{thebibliography}

